Joint Latent Class Trees: A Tree-Based Approach to Modeling Time-to-event and Longitudinal Data

In this paper, we propose a semiparametric, tree based joint latent class modeling approach (JLCT) to model the joint behavior of longitudinal and time-to-event data. Existing joint latent class modeling approaches are parametric and can suffer from high computational cost. The most common parametric approach, the joint latent class model (JLCM), further restricts analysis to using time-invariant covariates in modeling survival risks and latent class memberships. Instead, the proposed JLCT is fast to fit, and can use time-varying covariates in all of its modeling components. We demonstrate the prognostic value of using time-varying covariates, and therefore the advantage of JLCT over JLCM on simulated data. We further apply JLCT to the PAQUID data set and confirm its superior prediction performance and orders-of-magnitude speedup over JLCM.

==> biblatex-vancouver/README <==
                        BibLaTex Vancouver
			==================

This package provides the Vancouver reference style for BibLateX. It is based on
the numeric style and requires biber.

Downloading
-----------

Latest release of BibLaTeX Vancouver can be downloaded from
http://code.agnibho.com/biblatex-vancouver/


Installation
------------

Install the package to your local texmf directory. The local texmf directory can
be found by running 'kpsewhich -var-value TEXMFHOME' in the commandline.

For example if your local texmf directory is '~/texmf', then copy the
'biblatex-vancouver' folder to '~/texmf/tex/latex/'.

Usage
-----

BibLaTex Vancouver can be included in your LaTex document as a style argument.

Example:
    \usepackage[backend=biber,style=vancouver]{biblatex}

Acknowledgment
--------------

Some part of the code has been adapted from the biblatex-nejm package.

Licensing
---------

Copyright (c) 2020 Agnibho Mondal
All rights reserved

This file is part of BibLaTex Vancouver.

BibLaTex Vancouver is free software: you can redistribute it and/or modify it
under the terms of the GNU General Public License as published by the Free
Software Foundation, either version 3 of the License, or (at your option) any
later version.

BibLaTex Vancouver is distributed in the hope that it will be useful, but
WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE.  See the GNU General Public License for more
details.

You should have received a copy of the GNU General Public License along with
BibLaTex Vancouver.  If not, see <http://www.gnu.org/licenses/>.

Contact
--------

Agnibho Mondal
contact@agnibho.com
www.agnibho.com

